A multishift, multipole rational QZ method with aggressive early deflation

The rational QZ method generalizes the QZ method by implicitly supporting rational subspace iteration. In this paper we extend the rational QZ method by introducing shifts and poles of higher multiplicity in the Hessenberg pencil, which is a pencil consisting of two Hessenberg matrices. The result is a multishift, multipole iteration on block Hessenberg pencils which allows one to stick to real arithmetic for a real input pencil. In combination with optimally packed shifts and aggressive early deflation as an advanced deflation technique we obtain an efficient method for the dense generalized eigenvalue problem. In the numerical experiments we compare the results with state-of-the-art routines for the generalized eigenvalue problem and show that we are competitive in terms of speed and accuracy.

==> theory.tex <==
\section{Uniqueness and convergence}
\label{sec:theory}
In this section we motivate the implicit approach used in the
multishift, multipole RQZ step in the form of an implicit Q theorem for block
Hessenberg pencils.
We also discuss the subspace iteration that is implicitly performed during the multishift,
multipole RQZ step.

The following lemma first extends the essential uniqueness of the QR factorization
to a form of essential uniqueness in the factorization of a matrix as a product of
a unitary matrix and a block upper triangular matrix.

\begin{lemma}
\label{lemma:blockQR}
Given a nonsingular $n{\times}n$ matrix $A$ and consider $A = \hat{Q} \hat{R}_{\bm{s}}$,
$A = \check{Q} \check{R}_{\bm{s}}$ two block QR factorizations where $\hat{Q}, \check{Q}$
are unitary matrices and $\hat{R}_{\bm{s}}, \check{R}_{\bm{s}}$ are block upper triangular
matrices with the same partition $\bm{s} = (s_1,\hdots,s_m)$.
Then $\hat{Q} = \check{Q} D_{\bm{s}}$ with $D_{\bm{s}}$ a unitary block diagonal matrix
with an identical partition $\bm{s}$ as $\hat{R}_{\bm{s}}$ and $\check{R}_{\bm{s}}$.
\end{lemma}

\begin{proof}
From $\hat{Q} \hat{R}_{\bm{s}} = \check{Q} \check{R}_{\bm{s}}$ it follows that,
$
\check{Q}^* \hat{Q} = \check{R}_{\bm{s}} \hat{R}_{\bm{s}}^{-1} =  \tilde{R}_{\bm{s}} = D_{\bm{s}},
$
with $\tilde{R}_{\bm{s}}$ a unitary block upper triangular matrix with partition ${\bm{s}}$.
The only unitary block upper triangular matrices are block diagonal matrices $D_{\bm{s}}$.
\end{proof}

Before presenting the implicit Q theorem, we first give this direct corollary of 
\Cref{thm:blockHessspaces} that considers the structure of rational Krylov matrices
instead of the subspaces. This is the block generalization of \cite[Corollary 5.7]{camps2019rational}.

\begin{corollary}
\label{cor:blockHessmatrices}
Given an $n{\times}n$ proper block Hessenberg pencil $(A,B)$ with partition
$\bm{s} = (s_1$, $\hdots$, $s_m)$
and poles
$\Xi = (\Xi^1, \hdots, \Xi^m)$ that are different from the eigenvalues.
Then for a tuple of shifts
$\Rho$ different from the poles,
$
K^{\text{rat}}_n(A,B,\bm{e}_1,\Xi, \Rho)
$
is a full rank $n{\times}n$ block upper triangular matrix
with partition $(1,s_1, s_2,\hdots, s_m)$.
While,
$
L^{\text{rat}}_{n-1}(A,B,\bm{z}_1,(\breve{\Xi}^1, \Xi^2, \hdots, \Xi^m), \Rho)
$
is a full rank $n{\times}n{-}1$ block upper triangular matrix with partition 
$(s_1, s_2,\hdots, s_m)$.
Here $\bm{z}_1$ and $\breve{\Xi}^1$ are chosen as described
in \Cref{thm:blockHessspaces}.
\end{corollary}

We are now ready to state the block implicit Q theorem.

\begin{theorem}
\label{thm:implicitQ}
Let $(A,B)$ be a regular matrix pencil and let $\hat{Q}, \check{Q}, \hat{Z}, \check{Z}$
be unitary matrices with $\hat{Q}\bm{e}_1 = \sigma \check{Q} \bm{e}_1$, $|\sigma| = 1$,
such that,
\begin{equation*}
(\hat{A}, \hat{B}) = \hat{Q}^* (A,B) \hat{Z}
\quad \text{and} \quad
(\check{A}, \check{B}) = \check{Q}^* (A,B) \check{Z},
\end{equation*}
are both proper block Hessenberg pencils with the same partition $(s_1, \hdots, s_m)$
and poles $\Xi = (\Xi^1, \hdots, \Xi^m)$ different from the eigenvalues.
Then the pencils $(\hat{A}, \hat{B})$ and $(\check{A},\check{B})$ are identical
up to multiplication with two unitary block diagonal matrices,
\begin{align*}
\hat{A} = D^*_1 \check{A} D_2
\quad \text{and} \quad
\hat{B} = D^*_1 \check{B} D_2,
\end{align*}
with $D_1$ having partition $(1, s_1, \hdots, s_m)$ and $D_2$ having partition
$(s_1, \hdots, s_m, 1)$.
\end{theorem}


\begin{proof}
\Cref{cor:blockHessmatrices} states that
$K^{\text{rat}}_n(\hat{A},\hat{B},\bm{e}_1,\Xi, \Rho)$
and
$K^{\text{rat}}_n(\check{A},\check{B},\bm{e}_1,\Xi, \Rho)$
are both block upper triangular matrices of full rank with
block partition $(1,s_1, \hdots, s_m)$.
We thus have,
%
\begin{equation*}
\begin{split}
& \hat{Q} \, K_{n}^{\text{rat}}(\hat{A}, \hat{B}, \bm{e}_1, \Xi, \Rho) \\
%
= \ & \hat{Q} \, \left[ \bm{e}_1, \ \hat{M}(\varrho_1,\xi_1) \; \bm{e}_1,
\ \hdots, \
\left( \prod_{i=1}^{n-1} \hat{M}(\varrho_i,\xi_i) \right) \; \bm{e}_1 \right] \\
%
= \ & \hat{Q} \, \left[ \bm{e}_1, \ \hat{Q}^* M(\varrho_1,\xi_1) \hat{Q} \; \bm{e}_1,
\ \hdots, \
\hat{Q}^* \left( \prod_{i=1}^{n-1} M(\varrho_i,\xi_i) \right) \hat{Q} \; \bm{e}_1
\right] \\
%
= \ & \phantom{Q} \,  \left[ \hat{\bm{q}}_1, \ M(\varrho_1,\xi_1) \; \hat{\bm{q}}_1,
\ \hdots, \
\left( \prod_{i=1}^{n-1} M(\varrho_i,\xi_i) \right) \; \hat{\bm{q}}_1 \right] \\
%
= \ & \sigma \;  \left[ \check{\bm{q}}_1, \ M(\varrho_1,\xi_1) \; \check{\bm{q}}_1,
\ \hdots, \
\left( \prod_{i=1}^{n-1} M(\varrho_i,\xi_i) \right) \; \check{\bm{q}}_1 \right] \\
%
= \ & \sigma \check{Q} \, K_{n}^{\text{rat}}(\check{A},\check{B}, \bm{e}_1, \Xi,\Rho).
\end{split}
\end{equation*}
From \Cref{lemma:blockQR} we have that this equality between two block QR factorizations
implies that $\hat{Q} = \check{Q} D_{(1,s_1,\hdots,s_m)}$.
%
For the relation between $\hat{Z}$ and $\check{Z}$, consider,
\begin{equation*}
(\doublehat{A},\doublehat{B}) = \doublehat{Q}^* \, (\hat{A},\hat{B}) \, \doublehat{Z},
\quad \text{and,} \quad
(\doublecheck{A},\doublecheck{B}) = \doublecheck{Q}^* \, (\check{A},\check{B}) \, \doublecheck{Z},
\end{equation*}
both reductions of the block Hessenberg pencils to a proper Hessenberg pencil as defined in
\Cref{lemma:blockHessToHess} and assume, without loss of generality, that $\xi_{s_1}^1$ is the
first pole in both $(\doublehat{A},\doublehat{B})$ and $(\doublecheck{A},\doublecheck{B})$.
Thus $\doublehat{\bm{z}}_1$ is the right eigenvector of the pole pencil of
$(\doublehat{A},\doublehat{B})$ associated with the eigenvalue $\xi_{s_1}^1$ and the same
holds for $\doublecheck{\bm{z}}_1$ and $(\doublecheck{A},\doublecheck{B})$. This implies,
\begin{equation*}
\doublehat{Q}^* \, (\hat{A} - \xi_{s_1}^1 \hat{B}) \doublehat{\bm{z}}_1 = \hat{\gamma} \bm{e}_1 ,
\quad \text{and,} \quad
\doublecheck{Q}^* \, (\check{A} - \xi_{s_1}^1 \check{B}) \doublecheck{\bm{z}}_1 = \check{\gamma} \bm{e}_1,
\end{equation*}
by the proper Hessenberg structure of $(\doublehat{A},\doublehat{B})$ and
$(\doublecheck{A},\doublecheck{B})$. Since by \cref{eq:reduction},
$\doublehat{Q} \bm{e}_1 = \doublecheck{Q} \bm{e}_1 = \bm{e}_1$, we also have,
\begin{equation*}
(\hat{A} - \xi_{s_1}^1 \hat{B}) \doublehat{\bm{z}}_1 = \hat{\gamma} \bm{e}_1 ,
\quad \text{and,} \quad
(\check{A} - \xi_{s_1}^1 \check{B}) \doublecheck{\bm{z}}_1 = \check{\gamma} \bm{e}_1,
\end{equation*}
Thus,
\begin{equation*}
\hat{Q}^* (A - \xi_{s_1}^1 B) \hat{Z} \doublehat{\bm{z}}_1 = \hat{\gamma} \bm{e}_1,
\quad \text{and,} \quad
\check{Q}^* (A - \xi_{s_1}^1 B) \check{Z} \doublecheck{\bm{z}}_1 = \check{\gamma} \bm{e}_1.
\end{equation*}
Using,
$\hat{Q} = \check{Q} D_{(1,s_1,\hdots,s_m)}$, $D_{(1,s_1,\hdots,s_m)} \bm{e}_1 = \sigma \bm{e}_1$,
we get that,
\begin{equation*}
\begin{split}
\hat{Z} \doublehat{\bm{z}}_1 
&= \hat{\gamma} (A- \xi_{s_1}^1 B)^{-1} \check{Q} D_{(1,s_1,\hdots,s_m)} \bm{e}_1
= \sigma \hat{\gamma} (A- \xi_{s_1}^1 B)^{-1} \check{Q}\bm{e}_1 \\
\check{Z} \doublecheck{\bm{z}}_1
& = \check{\gamma} (A- \xi_{s_1}^1 B)^{-1} \check{Q} \bm{e}_1,
\end{split}
\end{equation*}
from which we conclude that
$\hat{Z} \doublehat{\bm{z}}_1 = \tilde{\sigma} \check{Z} \doublecheck{\bm{z}}_1$
for some $\tilde{\sigma}$ with $|\tilde{\sigma}| = 1$.
%
Now use this result in combination with \Cref{cor:blockHessmatrices},
\begin{equation*}
\begin{split}
& \hat{Z} \, L_{n-1}^{\text{rat}}(\hat{A}, \hat{B}, \doublehat{\bm{z}}_1, \Xi, \Rho) \\
%
= \ & \hat{Z} \, \left[ \doublehat{\bm{z}}_1, \ \hat{N}(\varrho_1,\xi_1) \; \doublehat{\bm{z}}_1,
\ \hdots, \
\left( \prod_{i=2}^{n-1} \hat{N}(\varrho_i,\xi_i) \right) \; \doublehat{\bm{z}}_1 \right] \\
%
= \ & \phantom{Z} \,  \left[\hat{Z}\doublehat{\bm{z}}_1 , \ N(\varrho_1,\xi_1) \; \hat{Z}\doublehat{\bm{z}}_1,
\ \hdots, \
\left( \prod_{i=2}^{n-1} N(\varrho_i,\xi_i) \right) \; \hat{Z}\doublehat{\bm{z}}_1 \right] \\
%
= \ & \tilde{\sigma} \;  \left[ \check{Z}\doublecheck{\bm{z}}_1, \ N(\varrho_1,\xi_1) \; \check{Z}\doublecheck{\bm{z}}_1,
\ \hdots, \
\left( \prod_{i=2}^{n-1} N(\varrho_i,\xi_i) \right) \; \check{Z}\doublecheck{\bm{z}}_1 \right] \\
%
= \ & \tilde{\sigma} \; \check{Z} \, L_{n-1}^{\text{rat}}(\check{A}, \check{B}, \doublecheck{\bm{z}}_1, \Xi, \Rho).
\end{split}
\end{equation*}
Based on \Cref{lemma:blockQR} we can now guarantee that the first $n{-}1$ columns of $\hat{Z}$ 
are equal to the first $n{-}1$ columns of $\check{Z}$ multiplied with some $n{-}1{\times}n{-}1$
unitary block diagonal matrix $D_{(s_1,\hdots,s_m)}$. Observe that this also determines 
$\hat{\bm{z}}_n = \breve{\sigma} \check{\bm{z}}_n$, $|\breve{\sigma}| = 1$.
This concludes the proof.
\end{proof}

In \cite[Theorem 6.1]{camps2019rational} it is shown that an RQZ step with shift $\varrho$
on a Hessenberg pencil with pole tuple $\Xi = (\xi_1, \hdots, \xi_{n-1})$ and new
pole $\xi_n$ performs nested subspace iteration accelerated by
\begin{equation}
q_{k}^{Q}(z) = \frac{z - \varrho}{z - \xi_k},
\quad \text{and} \quad
q_{k}^{Z}(z) = \frac{z - \varrho}{z - \xi_{k+1}},
\end{equation}
for the $k$th column vector of respectively $Q$ and $Z$. Based on \Cref{lemma:blockHessToHess},
this can be extended to block Hessenberg pencils under the condition that the partition
$\bm{s}$ prior to the multishift, multipole RQZ step is the same as the partition $\hat{\bm{s}}$
afterwards.
We omit this generalization as the condition  $\bm{s}= \hat{\bm{s}}$ limits the practical
application of the theoretical result.
Combining \cite[Theorem 6.1]{camps2019rational} with \Cref{lemma:blockHessToHess}, it is clear, however,
that in the multishift, multipole RQZ method shifts that have been swapped along the subdiagonal
of the block Hessenberg pencil will lead to deflations at the end of the pencil, while
poles that have been moved to the front of the pencil lead to convergence of eigenvalues at the
beginning. This holds under the assumption that a good choice of poles and shifts is made.


